Task Attended Meta-Learning for Few-Shot Learning

Meta-learning (ML) has emerged as a promising direction in learning models under constrained resource settings like few-shot learning. The popular approaches for ML either learn a generalizable initial model or a generic parametric optimizer through episodic training. The former approaches leverage the knowledge from a batch of tasks to learn an optimal prior. In this work, we study the importance of a batch for ML. Specifically, we first incorporate a batch episodic training regimen to improve the learning of the generic parametric optimizer. We also hypothesize that the common assumption in batch episodic training that each task in a batch has an equal contribution to learning an optimal meta-model need not be true. We propose to weight the tasks in a batch according to their "importance" in improving the meta-model's learning. To this end, we introduce a training curriculum motivated by selective focus in humans, called task attended meta-training, to weight the tasks in a batch. Task attention is a standalone module that can be integrated with any batch episodic training regimen. The comparisons of the models with their non-task-attended counterparts on complex datasets like miniImageNet and tieredImageNet validate its effectiveness.

==> Task-attended Metalearning /mybibliography.tex <==
\begin{thebibliography}{10}
\providecommand{\url}[1]{\texttt{#1}}
\providecommand{\urlprefix}{URL }
\providecommand{\doi}[1]{https://doi.org/#1}

\bibitem{andrychowicz2016learning}
Andrychowicz, M., Denil, M., Gomez, S., Hoffman, M.W., Pfau, D., Schaul, T.,
  Shillingford, B., De~Freitas, N.: Learning to learn by gradient descent by
  gradient descent. In: NeurIPS (2016)

\bibitem{DBLP:conf/iclr/AntoniouES19}
Antoniou, A., Edwards, H., Storkey, A.J.: How to train your {MAML}. In: {ICLR}
  (2019)

\bibitem{DBLP:conf/icml/ChenHCDLBF17}
Chen, Y., Hoffman, M.W., Colmenarejo, S.G., Denil, M., Lillicrap, T.P.,
  Botvinick, M., de~Freitas, N.: Learning to learn without gradient descent by
  gradient descent. In: {ICML} (2017)

\bibitem{DBLP:journals/tip/DasL20}
Das, D., Lee, C.S.G.: A two-stage approach to few-shot learning for image
  recognition. {IEEE} Trans. Image Process.  (2020)

\bibitem{DBLP:conf/icml/FinnAL17}
Finn, C., Abbeel, P., Levine, S.: Model-agnostic meta-learning for fast
  adaptation of deep networks. In: {ICML} (2017)

\bibitem{DBLP:conf/nips/FinnXL18}
Finn, C., Xu, K., Levine, S.: Probabilistic model-agnostic meta-learning. In:
  NeurIPS (2018)

\bibitem{hochreiter1997long}
Hochreiter, S., Schmidhuber, J.: Long short-term memory. Neural computation
  (1997)

\bibitem{DBLP:conf/nips/HouCMSC19}
Hou, R., Chang, H., Ma, B., Shan, S., Chen, X.: Cross attention network for
  few-shot classification. In: NeurIPS (2019)

\bibitem{DBLP:conf/cvpr/JamalQ19}
Jamal, M.A., Qi, G.: Task agnostic meta-learning for few-shot learning. In:
  {CVPR} (2019)

\bibitem{DBLP:journals/corr/KingmaB14}
Kingma, D.P., Ba, J.: Adam: {A} method for stochastic optimization. In: {ICLR}
  (2015)

\bibitem{koch2015siamese}
Koch, G., Zemel, R., Salakhutdinov, R.: Siamese neural networks for one-shot
  image recognition. In: ICML deep learning workshop (2015)

\bibitem{lake2015human}
Lake, B.M., Salakhutdinov, R., Tenenbaum, J.B.: Human-level concept learning
  through probabilistic program induction. Science  (2015)

\bibitem{DBLP:conf/cvpr/LeeMRS19}
Lee, K., Maji, S., Ravichandran, A., Soatto, S.: Meta-learning with
  differentiable convex optimization. In: {CVPR} (2019)

\bibitem{DBLP:journals/corr/LiZCL17}
Li, Z., Zhou, F., Chen, F., Li, H.: Meta-sgd: Learning to learn quickly for
  few-shot learning (2017)

\bibitem{DBLP:conf/iclr/MishraR0A18}
Mishra, N., Rohaninejad, M., Chen, X., Abbeel, P.: A simple neural attentive
  meta-learner. In: {ICLR} (2018)

\bibitem{munkhdalai2017meta}
Munkhdalai, T., Yu, H.: Meta networks. In: ICML

\bibitem{DBLP:journals/corr/abs-1803-02999}
Nichol, A., Achiam, J., Schulman, J.: On first-order meta-learning algorithms.
  CoRR  (2018)

\bibitem{DBLP:conf/nips/OreshkinLL18}
Oreshkin, B.N., L{\'{o}}pez, P.R., Lacoste, A.: {TADAM:} task dependent
  adaptive metric for improved few-shot learning. In: NeurIPS (2018)

\bibitem{rajeswaran2019meta}
Rajeswaran, A., Finn, C., Kakade, S.M., Levine, S.: Meta-learning with implicit
  gradients. In: NeurIPS (2019)

\bibitem{DBLP:conf/iclr/RaviL17}
Ravi, S., Larochelle, H.: Optimization as a model for few-shot learning. In:
  {ICLR} (2017)

\bibitem{DBLP:conf/iclr/RenTRSSTLZ18}
Ren, M., Triantafillou, E., Ravi, S., Snell, J., Swersky, K., Tenenbaum, J.B.,
  Larochelle, H., Zemel, R.S.: Meta-learning for semi-supervised few-shot
  classification. In: {ICLR} (2018)

\bibitem{santoro2016meta}
Santoro, A., Bartunov, S., Botvinick, M., Wierstra, D., Lillicrap, T.:
  Meta-learning with memory-augmented neural networks. In: ICML (2016)

\bibitem{DBLP:conf/nips/SnellSZ17}
Snell, J., Swersky, K., Zemel, R.S.: Prototypical networks for few-shot
  learning. In: {NeurIPS} (2017)

\bibitem{DBLP:journals/corr/abs-1910-03648}
Sun, Q., Liu, Y., Chen, Z., Chua, T., Schiele, B.: Meta-transfer learning
  through hard tasks. CoRR  (2019)

\bibitem{DBLP:conf/cvpr/SunLCS19}
Sun, Q., Liu, Y., Chua, T., Schiele, B.: Meta-transfer learning for few-shot
  learning. In: {CVPR} (2019)

\bibitem{DBLP:conf/cvpr/SungYZXTH18}
Sung, F., Yang, Y., Zhang, L., Xiang, T., Torr, P.H.S., Hospedales, T.M.:
  Learning to compare: Relation network for few-shot learning. In: {CVPR}
  (2018)

\bibitem{vinyals2016matching}
Vinyals, O., Blundell, C., Lillicrap, T., Wierstra, D., et~al.: Matching
  networks for one shot learning. In: NeurIPS (2016)

\bibitem{DBLP:conf/icml/WichrowskaMHCDF17}
Wichrowska, O., Maheswaranathan, N., Hoffman, M.W., Colmenarejo, S.G., Denil,
  M., de~Freitas, N., Sohl{-}Dickstein, J.: Learned optimizers that scale and
  generalize. In: {ICML} (2017)

\bibitem{DBLP:conf/nips/ZhangCGBS18}
Zhang, R., Che, T., Ghahramani, Z., Bengio, Y., Song, Y.: Metagan: An
  adversarial approach to few-shot learning. In: NeurIPS (2018)

\bibitem{DBLP:journals/corr/abs-2007-06240}
Zhou, Y., Wang, Y., Cai, J., Zhou, Y., Hu, Q., Wang, W.: Expert training: Task
  hardness aware meta-learning for few-shot classification. CoRR  (2020)

\end{thebibliography}

